Towards a Personal Health Knowledge Graph Framework for Patient Monitoring

Healthcare providers face significant challenges with monitoring and managing patient data outside of clinics, particularly with insufficient resources and limited feedback on their patients' conditions. Effective management of these symptoms and exploration of larger bodies of data are vital for maintaining long-term quality of life and preventing late interventions. In this paper, we propose a framework for constructing personal health knowledge graphs from heterogeneous data sources. Our approach integrates clinical databases, relevant ontologies and standard healthcare guidelines to support alert generation, clinician interpretation and querying of patient data. Through a use case of monitoring Chronic Obstructive Pulmonary Disease (COPD) patients, we demonstrate that inference and reasoning on personal health knowledge graphs built with our framework can aid in patient monitoring and enhance the efficacy and accuracy of patient data queries.

==> body_archive.tex <==
abstract


%Healthcare providers have challenges with monitoring and navigating patient data adequately outside of clinic due to poor options and opportunities for feedback and data of their condition. Proper management of these symptoms and exploring larger bodies of data effectively are vital in maintaining the quality of life and comfort for the sufferers long-term, and reducing the risk of providing healthcare too late. We propose a knowledge graph composed to support clinicians' ability to interpret and query patient data for tasks such as monitoring and cohort selection. Data extracted from the MIMIC-III clinical database of ICU patients was used to test rule-based and machine learning inference features, created from expert knowledge and statistical modelling. The results of our work so far suggest that inference and reasoning over data in a knowledge graph containing adequate expert knowledge can be used to aid in the remote monitoring of patients and effective selection for patient care


introduction

%and even create subgraphs in patient querying through extracting the relationships and nodes within a query over the data, both aiding in clear specific visualisations and efficiency. They also provide the necessary connections and relationships between the terminology to provide appropriate context within the domain model, which then augments the patient data for a broader understanding and interpretation. As digital healthcare solutions become more prevalent, so to will the need for a formal reference of the healthcare discoveries to date and how to apply them to digital health records and patient data for powerful insights. 

%Clinicians and sufferers alike have challenges related to the ability to appropriately monitor the symptoms of chronic disease within the sufferer. Clinicians are reliant on direct interactions with the sufferer, which can be challenging to arrange when there are other clinical matters to attend to. This would indicate a need for solutions that can allow clinicians to monitor the sufferers when they are outside of clinic. The solution we propose will provide actionable insights and alerts based on expert knowledge and support from both rule-based and model-based inference approaches. The intended benefits of this system are to aid in clinical decision making for prompting both arranging consultations with patients and/or providing urgent care where necessary.


%\subsection{Objective}

%The challenge we wish to focus on in this paper is related to the data management and interpretation of the data. ?
%The data in question will be the monitoring data from the device in contact or the vicinity of the sufferer, and any additional data provided by healthcare providers. These data will be collected from different sources and a combination of continuous and sessional forms, which will also be required to be modular for potential other devices being featured in the system. 

%The component of this pipeline that we wish to tackle with the discussed work in this paper will be aiming to solve the data management, interpretation, and reasoning over the data for responding to considerably developing symptoms. Due to the complications and difficulty involved in collecting appropriate data for training a model for this task, an expert knowledge based approach is proposed, which will learn and adapt with both the expert knowledge being updated and the data from the sufferer allowing a personalization of the system's understanding of the condition and symptoms.



%\subsection{Personalised Health Knowledge Graph}
% Personalised health knowledge graphs are sophisticated data structures that represent medical concepts and the relationships between them, allowing researchers to integrate and analyze patient data from various sources, including EHRs, claims, and unstructured clinical notes. They are powerful ways to link domain knowledge and the relevant terminology with clinical data for patients, and even create subgraphs in patient querying through extracting the relationships and nodes within a query over the data, both aiding in clear specific visualisations and efficiency. They also provide the necessary connections and relationships between the terminology to provide appropriate context within the domain model, which then augments the patient data for a broader understanding and interpretation. As digital healthcare solutions become more prevalent, so to will the need for a formal reference of the healthcare discoveries to date and how to apply them to digital health records and patient data for powerful insights. 
 
%\subsection{Related Works}
%In 2018, Gyrard et al.\cite{phkg} published about the challenges of creating PHKGs that adequately ``synthesize and deduce meaningful information embodying the vision of the Data, Information, Knowledge, and Wisdom (DIKW) pyramid'', and propose a solution combining IoT data analytics and explicit knowledge upon 3 chronic disease use cases. %They express that there is a lack of appropriate exploitation of contextual data, personalized data and integration with background medical knowledge bases in monitoring user health, and that personalized knowledge graphs are possible solutions to these shortcomings in our current approaches to monitoring in healthcare. 
%Their solution combines electronic health records (EHR), environmental data and personal health signals, then integrate domain knowledge from relevant ontologies to annotate the datasets. Following this integration, a proposed rule-based reasoning engine can then be applied the deduce ``meaningful insights from heterogeneous data''. They describe ``sketching'' their solution, implying that the solution is theoretical. We aim to actualise a similar solution to what they have described.
%The work described this paper is related to the data management and interpretation of patient data. These data will be collected from different sources and a combination of continuous and sessional data. 
%Several projects of related work have featured NoSQL (such as MongoDB), ODBA (Ontology-Based Data Access) solutions, and similarly ontology based data integration, which describes an approach to bringing data sources together. An example is Araujo, et al.\cite{ontomongo}, who proposed their solution called OntoMongo, which builds from the discussions of \cite{Botoeva2016OBDABR} in their paper regarding OBDA beyond relational databases. Their solution is to use ontological mappings to data in the database, however querying with SPARQL from the ontology side towards the data. RDF and SPARQL can have limitations of expression in both the flexibility of schema and the querying of the format. Label property graphs have benefits in ease of understanding of the Cypher syntax and ways to easily express the nodes and relationships between them, and the ability to define more information within the nodes and relationships in the graph itself. %, their rationale being that being able to integrate these separate approaches to NoSQL data storage is vital as a response to the developments of the World Wide Web infrastructure. 

%We wish to already have a knowledge graph/ontology created that features the physical health and COPD's clinical vocabulary ready for mapping with. The integration with other tooling in our overall use case also incentivized approaching querying and reasoning with the data as the start point rather than the ontology and not use SPARQL for the querying solution.

data

%The solution is designed to be as independent of specific sources as possible, however the example dataset that was used as an example for implementing the appropriate components for the pipeline and processing was MIMIC-III\cite{mimiciii}, a large freely accessible database featuring anonymized data on patients admitted to critical care units at a large tertiary care hospital. This gave us a large multi-modal dataset of vital sign measurements, notes and other unstructured data and patients to work through the tool with varying symptom severity to test the alert generation at the end of the pipeline, while providing a use case of challenges in how to manage the data.

proposed framework and implementation
%In this section, we describe the components of the flow through the COPH knowledge graph, including the relationship with data sources, the mapping of the data to the semantic terms within the ontology, and finally the alert system based on the resulting relationships from the generated instances from the representations of the data and patients within the knowledge graph.


semantic mapping
%The mappings were be stored in MongoDB and could be queried and returned using the measurement type stored within the measurement document's context fields.
Using this,% we then have an intermediate processing stage between MongoDB and the knowledge graph that allows us to 

time series data summarization
%The summaries of the measurements are splitting a day into quarters, IE. a summary for each 6 hours of the day. This is easy to achieve as appropriate summary statistics that can be calculated and then uploaded within the upload tool into MongoDB. Different summary statistics had to be implemented to deal with different data types, for example numerical data could use averaging, however that becomes challenging with string data, and as such an alternative was found in "Most common", which will then use the most commonly found string in the data as the summary value. Timestamps are stored typically as properties and can be accessed easily through queries and smart filters can be applied using comparisons with other dates (for example, any date before another date).

%\subsection{Scoring and Alerts}

%We take the measurements, pre-process them ready for the scoring systems, score them based on thresholds either general or personalised for the patient, and then generate alerts from the scores. An additional Kolmogorov Smirnov test is conducted as an alert generation method from the time-series comparison with historical data, comparing the distribution of the most recent 3 days of the patient's measurements with the rest of the month before it. This comparison helps to understand whether something concerning may be happening with the patient's symptoms acutely.

risk scoring 
%The selection of appropriate patient cohorts is a crucial aspect of medical research and clinical trials. Researchers require a representative sample of patients that meet specific criteria, such as age, gender, disease severity, and comorbidities, among other factors, to ensure that their findings are accurate and generalizable. However, the process of selecting suitable patient cohorts can be time-consuming, complex, and error-prone, particularly when dealing with large volumes of structured and unstructured patient data.

%To address this challenge, we proposed to use of a personal health knowledge graph. 

%We utilized the Medical Concept Annotation Toolkit (MedCAT), which is an open-source library providing Named Entity Recognition and Linking (NER+L) functionalities, as well as an annotation tool and an online learning training interface. \cite{MedCAT}.

%Initially, we extracted information from MIMIC III patient’s note and conducted preliminary statistical analysis, including calculating document count per patient and age-based statistics. Next, we installed MedCAT version 1.5.0 on our Jupyter notebook and configured three key components - vocab, concept database (CDB), and CDB configuration - to utilize the MedCat model.

%The vocab model has two primary functions, spell checking and word embedding. It comprises token, wordcounts, and vector embedding, which can be pre-calculated using word2vec or BERT. To build the concept database, we created a custom database by using the Snomed CT ontology to develop a list of all concepts we wanted to detect and link to. The CDB configuration was tailored to our specific use case, although the default configuration is adequate for most use cases.

%All three components were then combined to create a MedCat model pack. We performed self-supervised training on the raw document to train the MedCat models and annotate documents to obtain NER+L. Subsequently, the resulting output document from MedCat was imported into a graph database (Neo4j) using Cypher import queries.
 
 %Our queries were parameterized to retrieve patients who are appropriate for a particular cohort. By incorporating medical domain expertise and patient information into a graph database.

 harmonising multimodal

 %Medical data is complex and heterogeneous, often consisting of data from different modalities, such as imaging data, electronic health records, and Omics data such as genomics, metabolomics, transcriptomics and proteomics. Clinical multimodal data integration has the potential to provide a more comprehensive and accurate understanding of patient health, which can lead to more effective and personalized treatments.

%Integrating clinical data from multiple sources is a challenging task due to the heterogeneity of the data. The data are collected using different instruments, methods, and formats, making it difficult to integrate. For instance, imaging data can be acquired using various scanners or imaging protocols, resulting in differences in image quality and features. Electronic health records may contain different types of data, such as text notes, structured data, and unstructured data, which require different processing methods. Multimodal data integration methods must consider these differences and be capable of effectively integrating data from various modalities.

%There are different approaches to integrating multimodal clinical data, including model-based, rule-based, and data-driven approaches. Model-based approaches involve building a model that describes the relationship between different types of data and using this model to integrate the data. Rule-based approaches entail using expert knowledge to define rules for integrating the data. On the other hand, data-driven approaches involve using machine learning algorithms to discover patterns and relationships in the data and use this knowledge to integrate the data.

%- Semantic summarization based on classical clinical report, 
%- embeddings created using pretrained models for multimodal integration such as clinical LLMs. Ready for indexing or machine learning model/similarity based inferences. 

%\subsection{Semantic Mapping}


%\subsection{Reasoning and Inference}

%An example use case of reasoning would be to infer that a query should return the phenotypes of a condition in addition to the condition itself based on the subclass relationships.

data storage
%This was important to easily support many sources of data that gives the user power to focus less on restructuring the data and more on ensuring that, as long as the mappings were provided to understand the data, then processing could be done later as needed. 

%The approach to storing data in Neo4j is the temporal PHKGs, and the transformed and annotated data % to primarily summarise the data, specifically summarising the time series data in periods (for example, 1 summary per quarter of a day) 

results 
%To explore the available functionality to support inferring from the data and augmenting queries, we can utilise the expert knowledge featured in the ontology that are semantically mapped to the patient data. An example query could use subclasses of the terms to return additional results that were not explicitly stated. For example, we can query the data using an ICD9 code of a more general condition to not only return results for the ICD9 code provided, but also the subclasses of that condition, even when they do not have the queried condition. 

%This is not possible without inferences, as a standard query would instead only return patients with the diagnosis referenced via the ICD9 code given.

conclusion
%We have combined expert knowledge in the form of ontology for semantic mapping with patient data that, via the mappings to the data provided, can successfully infer for additional context and support clinical decision making. We have shown that knowledge graphs can be powerful assistance in providing support for healthcare providers to keep updated with changed patient context and make correct decisions for patient care and cohort selection.




